Stability analysis of thermo-acoustic nonlinear eigenproblems in annular combustors. Part I. Sensitivity

We present an adjoint-based method for the calculation of eigenvalue perturbations in nonlinear, degenerate and non self-adjoint eigenproblems. This method is applied to a thermo-acoustic annular combustor network, the stability of which is governed by a nonlinear eigenproblem. We calculate the first- and second-order sensitivities of the growth rate and frequency to geometric, flow and flame parameters. Three different configurations are analysed. The benchmark sensitivities are obtained by finite difference, which involves solving the nonlinear eigenproblem at least as many times as the number of parameters. By solving only one adjoint eigenproblem, we obtain the sensitivities to any thermo-acoustic parameter, which match the finite-difference solutions at much lower computational cost.

==> elsarticle.tex <==
%%
%% This file will generate fast loadable files and documentation
%% driver files from the doc files in this package when run through
%% LaTeX or TeX.
%%
%% Copyright 2007, 2008, 2009 Elsevier Ltd
%%
%% This file is part of the 'Elsarticle Bundle'.
%% ---------------------------------------------
%%
%% It may be distributed under the conditions of the LaTeX Project Public
%% License, either version 1.2 of this license or (at your option) any
%% later version.  The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%% and version 1.2 or later is part of all distributions of LaTeX
%% version 1999/12/01 or later.
%%
%% The list of all files belonging to the 'Elsarticle Bundle' is
%% given in the file 'manifest.txt'.
%%
%%
%%
\input docstrip.tex
%%\keepsilent

\preamble

Copyright 2007, 2008, 2009 Elsevier Ltd

This file is part of the 'Elsarticle Bundle'.
-------------------------------------------

It may be distributed under the conditions of the LaTeX Project Public
License, either version 1.2 of this license or (at your option) any
later version.  The latest version of this license is in
   http://www.latex-project.org/lppl.txt
and version 1.2 or later is part of all distributions of LaTeX
version 1999/12/01 or later.

The list of all files belonging to the 'Elsarticle Bundle' is
given in the file `manifest.txt'.

\endpreamble

\askforoverwritefalse

\generate{\file{elsarticle.cls}{\from{elsarticle.dtx}{class}}}
\obeyspaces
\Msg{*************************************************************}
\Msg{*                                                           *}
\Msg{* To finish the installation you have to move the following *}
\Msg{* file into a directory searched by TeX:                    *}
\Msg{*                                                           *}
\Msg{*     elsarticle.cls                                        *}
\Msg{*         and                                               *}
\Msg{*     elsarticle-*.bst                                      *}
\Msg{*                                                           *}
\Msg{* To produce the documentation go to the ../contrib folder  *}
\Msg{* and run the file elsdoc.tex through pdfLaTeX              *}
\Msg{* or use the Makefile which is far more easier.             *}
\Msg{*                                                           *}
\Msg{* Happy TeXing!                                             *}
\Msg{*                                                           *}
\Msg{*************************************************************}

\endbatchfile

